Channel Estimation for Diffusive Molecular Communications

In molecular communication (MC) systems, the \textit{expected} number of molecules observed at the receiver over time after the instantaneous release of molecules by the transmitter is referred to as the channel impulse response (CIR). Knowledge of the CIR is needed for the design of detection and equalization schemes. In this paper, we present a training-based CIR estimation framework for MC systems which aims at estimating the CIR based on the \textit{observed} number of molecules at the receiver due to emission of a \textit{sequence} of known numbers of molecules by the transmitter. Thereby, we distinguish two scenarios depending on whether or not statistical channel knowledge is available. In particular, we derive maximum likelihood (ML) and least sum of square errors (LSSE) estimators which do not require any knowledge of the channel statistics. For the case, when statistical channel knowledge is available, the corresponding maximum a posteriori (MAP) and linear minimum mean square error (LMMSE) estimators are provided. As performance bound, we derive the classical Cramer Rao (CR) lower bound, valid for any unbiased estimator, which does not exploit statistical channel knowledge, and the Bayesian CR lower bound, valid for any unbiased estimator, which exploits statistical channel knowledge. Finally, we propose optimal and suboptimal training sequence designs for the considered MC system. Simulation results confirm the analysis and compare the performance of the proposed estimation techniques with the respective CR lower bounds.

==> Fig/ISI/ISI.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextA b)}%
\psfrag{001}[bc][bc]{\matlabtextA Expected number of observed molecules}%
\psfrag{002}[tc][tc]{\matlabtextA Time (ms)}%
\psfrag{003}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}Desired\\Component\end{tabular}}%
\psfrag{004}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}ISI\\Components\end{tabular}}%
%
%% </text>

==> Fig/Mean_K/Mean_K.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA LMMSE Estimation\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA MAP Estimation\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA Suboptimal LSSE Estimation\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA Suboptimal ML Estimation\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA LSSE Estimation\hspace{0.5em}}%
\psfrag{024}[cl][cl]{\matlabtextA ML Estimation\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB Estimation Error Mean in dB}%
\psfrag{026}[tc][tc]{\matlabtextB Sequence Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $50$}%
\psfrag{005}[ct][ct]{\matlabtextC $60$}%
\psfrag{006}[ct][ct]{\matlabtextC $70$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $90$}%
\psfrag{009}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-16$}%
\psfrag{011}[rc][rc]{\matlabtextC $-14$}%
\psfrag{012}[rc][rc]{\matlabtextC $-12$}%
\psfrag{013}[rc][rc]{\matlabtextC $-10$}%
\psfrag{014}[rc][rc]{\matlabtextC $-8$}%
\psfrag{015}[rc][rc]{\matlabtextC $-6$}%
\psfrag{016}[rc][rc]{\matlabtextC $-4$}%
\psfrag{017}[rc][rc]{\matlabtextC $-2$}%
\psfrag{018}[rc][rc]{\matlabtextC $0$}%
%
%% </ytick>

==> Fig/Seq_LSSE/Seq_LSSE.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA ISI-Free Seq., Simp. Est., Sim. Result\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA ISI-Free Seq., LSSE Est., Sim. Result\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA Opt. Seq., LSSE Est., Sim. Result\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA ISI-Free Seq., LSSE Est., Analyt. Upp. Bound\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA Opt. Seq., LSSE Est., Analyt. Upp. Bound\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextB $L=5$}%
\psfrag{021}[cl][cl]{\matlabtextB $L=4$}%
\psfrag{022}[cl][cl]{\matlabtextB $L=3$}%
\psfrag{023}[cl][cl]{\matlabtextB $L=2$}%
\psfrag{024}[cl][cl]{\matlabtextB $L=1$}%
\psfrag{025}[bc][bc]{\matlabtextB Normalized Estimation Error Variance, $ \overline{\mathrm{Var}}_{\mathbf{e}}$, in dB}%
\psfrag{026}[tc][tc]{\matlabtextB Sequence Length $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $2$}%
\psfrag{001}[ct][ct]{\matlabtextC $4$}%
\psfrag{002}[ct][ct]{\matlabtextC $6$}%
\psfrag{003}[ct][ct]{\matlabtextC $8$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $12$}%
\psfrag{006}[ct][ct]{\matlabtextC $14$}%
\psfrag{007}[ct][ct]{\matlabtextC $16$}%
\psfrag{008}[ct][ct]{\matlabtextC $18$}%
\psfrag{009}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-25$}%
\psfrag{011}[rc][rc]{\matlabtextC $-20$}%
\psfrag{012}[rc][rc]{\matlabtextC $-15$}%
\psfrag{013}[rc][rc]{\matlabtextC $-10$}%
\psfrag{014}[rc][rc]{\matlabtextC $-5$}%
%
%% </ytick>

==> Fig/Seq_MMSE/Seq_MMSE.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextA ISI-Free Seq., Simp. Est., Sim. Result\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA ISI-Free Seq., LMMSE Est., Sim. Result\hspace{0.5em}}%
\psfrag{024}[cl][cl]{\matlabtextA Opt. Seq., LMMSE Est., Sim. Result\hspace{0.5em}}%
\psfrag{025}[cl][cl]{\matlabtextA ISI-Free Seq., LMMSE Est., Analyt. Upp. Bound\hspace{0.5em}}%
\psfrag{026}[cl][cl]{\matlabtextA Opt. Seq., LMMSE Est., Analyt. Upp. Bound\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{027}[cl][cl]{\matlabtextB $L=5$}%
\psfrag{028}[cl][cl]{\matlabtextB $L=3$}%
\psfrag{029}[cl][cl]{\matlabtextB $L=1$}%
\psfrag{030}[bc][bc]{\matlabtextB Normalized Estimation Error Variance, $ \overline{\mathrm{Var}}_{\mathbf{e}}$, in dB}%
\psfrag{031}[tc][tc]{\matlabtextB Sequence Length $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $2$}%
\psfrag{001}[ct][ct]{\matlabtextC $4$}%
\psfrag{002}[ct][ct]{\matlabtextC $6$}%
\psfrag{003}[ct][ct]{\matlabtextC $8$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $12$}%
\psfrag{006}[ct][ct]{\matlabtextC $14$}%
\psfrag{007}[ct][ct]{\matlabtextC $16$}%
\psfrag{008}[ct][ct]{\matlabtextC $18$}%
\psfrag{009}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-28$}%
\psfrag{011}[rc][rc]{\matlabtextC $-26$}%
\psfrag{012}[rc][rc]{\matlabtextC $-24$}%
\psfrag{013}[rc][rc]{\matlabtextC $-22$}%
\psfrag{014}[rc][rc]{\matlabtextC $-20$}%
\psfrag{015}[rc][rc]{\matlabtextC $-18$}%
\psfrag{016}[rc][rc]{\matlabtextC $-16$}%
\psfrag{017}[rc][rc]{\matlabtextC $-14$}%
\psfrag{018}[rc][rc]{\matlabtextC $-12$}%
\psfrag{019}[rc][rc]{\matlabtextC $-10$}%
\psfrag{020}[rc][rc]{\matlabtextC $-8$}%
\psfrag{021}[rc][rc]{\matlabtextC $-6$}%
%
%% </ytick>

==> Fig/Var_K/Var_K.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA LMMSE Estimation\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA MAP Estimation\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA Bayesian CR Bound\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA Suboptimal LSSE Estimation\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA Suboptimal ML Estimation\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA LSSE Estimation\hspace{0.5em}}%
\psfrag{024}[cl][cl]{\matlabtextA ML Estimation\hspace{0.5em}}%
\psfrag{025}[cl][cl]{\matlabtextA Classical CR Bound\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{026}[bc][bc]{\matlabtextB Estimation Error Variance in dB}%
\psfrag{027}[tc][tc]{\matlabtextB Sequence Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $50$}%
\psfrag{005}[ct][ct]{\matlabtextC $60$}%
\psfrag{006}[ct][ct]{\matlabtextC $70$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $90$}%
\psfrag{009}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $8$}%
\psfrag{011}[rc][rc]{\matlabtextC $10$}%
\psfrag{012}[rc][rc]{\matlabtextC $12$}%
\psfrag{013}[rc][rc]{\matlabtextC $14$}%
\psfrag{014}[rc][rc]{\matlabtextC $16$}%
\psfrag{015}[rc][rc]{\matlabtextC $18$}%
\psfrag{016}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $22$}%
%
%% </ytick>

==> Fig/Var_K_CIR/Var_K_CIR.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA LMMSE Estimation\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA LSSE Estimation\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextB $\sigma^2=[0.01,0.05,0.1,0.5,1]$}%
\psfrag{023}[bc][bc]{\matlabtextB Estimation Error Variance in dB}%
\psfrag{024}[tc][tc]{\matlabtextB Sequence Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $50$}%
\psfrag{005}[ct][ct]{\matlabtextC $60$}%
\psfrag{006}[ct][ct]{\matlabtextC $70$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $90$}%
\psfrag{009}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $4$}%
\psfrag{011}[rc][rc]{\matlabtextC $6$}%
\psfrag{012}[rc][rc]{\matlabtextC $8$}%
\psfrag{013}[rc][rc]{\matlabtextC $10$}%
\psfrag{014}[rc][rc]{\matlabtextC $12$}%
\psfrag{015}[rc][rc]{\matlabtextC $14$}%
\psfrag{016}[rc][rc]{\matlabtextC $16$}%
\psfrag{017}[rc][rc]{\matlabtextC $18$}%
\psfrag{018}[rc][rc]{\matlabtextC $20$}%
\psfrag{019}[rc][rc]{\matlabtextC $22$}%
%
%% </ytick>

==> Fig/Var_K_L/Var_K_L.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA LMMSE Estimation\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA LSSE Estimation\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextB $L=[1,2,3,4,5]$}%
\psfrag{020}[bc][bc]{\matlabtextB Normalized Estimation Error Variance, $ \overline{\mathrm{Var}}_{\mathbf{e}}$, in dB}%
\psfrag{021}[tc][tc]{\matlabtextB Sequence Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $50$}%
\psfrag{005}[ct][ct]{\matlabtextC $60$}%
\psfrag{006}[ct][ct]{\matlabtextC $70$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $90$}%
\psfrag{009}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-35$}%
\psfrag{011}[rc][rc]{\matlabtextC $-30$}%
\psfrag{012}[rc][rc]{\matlabtextC $-25$}%
\psfrag{013}[rc][rc]{\matlabtextC $-20$}%
\psfrag{014}[rc][rc]{\matlabtextC $-15$}%
\psfrag{015}[rc][rc]{\matlabtextC $-10$}%
\psfrag{016}[rc][rc]{\matlabtextC $-5$}%
%
%% </ytick>
